Lang-n-Send Extended: Sending Regular Expressions to Monitors

In prior work, Cimini has presented Lang-n-Send, a pi-calculus with language definitions. In this paper, we present an extension of this calculus called Lang-n-Send+m. First, we revise Lang-n-Send to work with transition system specifications rather than its language specifications. This revision allows the use of negative premises in deduction rules. Next, we extend Lang-n-Send with monitors and with the ability of sending and receiving regular expressions, which then can be used in the context of larger regular expressions to monitor the execution of programs. We present a reduction semantics for Lang-n-Send+m, and we offer examples that demonstrate the scenarios that our calculus captures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, L. Safina \& A. Scalas (Eds.):\\
15th Interaction and Concurrency Experience (ICE 2022)\\
EPTCS 365, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.365.5}{10.4204/EPTCS.365.5}}

